RANRAC: Robust Neural Scene Representations via Random Ray Consensus

Learning-based scene representations such as neural radiance fields or light field networks, that rely on fitting a scene model to image observations, commonly encounter challenges in the presence of inconsistencies within the images caused by occlusions, inaccurately estimated camera parameters or effects like lens flare. To address this challenge, we introduce RANdom RAy Consensus (RANRAC), an efficient approach to eliminate the effect of inconsistent data, thereby taking inspiration from classical RANSAC based outlier detection for model fitting. In contrast to the down-weighting of the effect of outliers based on robust loss formulations, our approach reliably detects and excludes inconsistent perspectives, resulting in clean images without floating artifacts. For this purpose, we formulate a fuzzy adaption of the RANSAC paradigm, enabling its application to large scale models. We interpret the minimal number of samples to determine the model parameters as a tunable hyperparameter, investigate the generation of hypotheses with data-driven models, and analyze the validation of hypotheses in noisy environments. We demonstrate the compatibility and potential of our solution for both photo-realistic robust multi-view reconstruction from real-world images based on neural radiance fields and for single-shot reconstruction based on light-field networks. In particular, the results indicate significant improvements compared to state-of-the-art robust methods for novel-view synthesis on both synthetic and captured scenes with various inconsistencies including occlusions, noisy camera pose estimates, and unfocused perspectives. The results further indicate significant improvements for single-shot reconstruction from occluded images. Project Page: https://bennobuschmann.com/ranrac/

==> figures/lfn_failure.tex <==
\begin{figure}
    \setlength\tabcolsep{0pt}
    \centering
    \begin{tabular}{cc cc cc cc cc}
    \includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/22d0561f06900e165140beb2199de2af.png}
    &
    \hspace{-0.01\textwidth}\includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/22d0561f06900e165140beb2199de2af_000006.png}
 & 
 \hspace{0.01\textwidth}
    &
    \includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/2c76aaa00e55c26836c07750784b6bc6.png}
    &
    \hspace{-0.02\textwidth}    \includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/2c76aaa00e55c26836c07750784b6bc6_000004.png}
 & 
 \hspace{0.02\textwidth}
    &
    \includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/4dc7fe6e98c4db21d79b19c7c4f0e293.png}
    &
    \hspace{-0.02\textwidth}    \includegraphics[width=0.085\textwidth]{images/lfn_failure_cases/4dc7fe6e98c4db21d79b19c7c4f0e293_000015.png}
    \\
    \end{tabular}
    \caption{Occlusion of important shape details (left, center) or perceptually-important elements (right) can lead to degenerate results. This mostly occurs for the chair class.}
    \label{fig:enter-label}
\end{figure}

==> figures/nerf_confusion.tex <==
% \begin{wrapfigure}{l}{0.3\textwidth}
    % \centering

\begin{table}[]
    \scriptsize
    \centering
    \setlength\tabcolsep{0pt}
    \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{>{\centering\arraybackslash} m{.4cm} >{\centering\arraybackslash} m{1.0cm} | >{\centering\arraybackslash} m{1cm} >{\centering\arraybackslash} m{1cm} | >{\centering\arraybackslash} m{0.5cm} }

\multicolumn{2}{c}{}&\multicolumn{2}{c}{Consensus Mild}&\\
% \cline{3-4}
\multicolumn{2}{c|}{}&Inlier&Outlier&\multicolumn{1}{c}{$\Sigma$}\\
\cline{2-5}
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Truth}}} & Inlier & \cellcolor[HTML]{339933} 108 & \cellcolor[HTML]{CCFFCC} 0 & 108 \\
% \cline{2-4}
& Outlier & \cellcolor[HTML]{CCFFCC} 0 & \cellcolor[HTML]{339933} 12 & 12\\
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{$\Sigma$} & \multicolumn{1}{c}{108} & \multicolumn{    1}{c|}{12} & \multicolumn{1}{c}{120}
\end{tabular}
\begin{tabular}{>{\centering\arraybackslash} m{.4cm} >{\centering\arraybackslash} m{1.0cm} | >{\centering\arraybackslash} m{1cm} >{\centering\arraybackslash} m{1cm} | >{\centering\arraybackslash} m{0.5cm} }

\multicolumn{2}{c}{}&\multicolumn{2}{c}{Consensus Heavy}&\\
% \cline{3-4}
\multicolumn{2}{c|}{}&Inlier&Outlier&\multicolumn{1}{c}{$\Sigma$}\\
\cline{2-5}

% \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Truth}}} &

{} &

Inlier & \cellcolor[HTML]{339933} 105 & \cellcolor[HTML]{FFFFC8} 
3 & 108 \\
% \cline{2-4}
& Outlier & \cellcolor[HTML]{FFFFC8} 2 & \cellcolor[HTML]{339933} 21 & 23\\
\cline{2-5}
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{$\Sigma$} & \multicolumn{1}{c}{107} & \multicolumn{1}{c|}{24} & \multicolumn{1}{c}{131}
    \end{tabular}
    % \vspace{-.25cm}
    \caption{The confusion matrices of RANRAC on the Watering Pot dataset show the successful elimination of occluded perspectives from the reconstruction. On the milder distracted dataset (left), all outliers and inliers are correctly labeled, resulting in a completely clean set of images. For the heavier distracted dataset (right), a very decent reconstruction is still possible, as only a minor amount of inconsistencies is mislabeled.}
    \label{tab:nerf_conf_matrix}
    % \vspace{-.5cm}
\end{table}
% \end{figure}
% \end{wrapfigure}

==> figures/nerf_qual.tex <==
% \begin{figure}
% \setlength\tabcolsep{0pt}
% \tiny
% \begin{tabular}{>{\centering\arraybackslash} m{1.8cm} >{\centering\arraybackslash} m{2.2cm} >{\centering\arraybackslash} m{2.2cm} >{\centering\arraybackslash} m{2.2cm}}
%     Ground Truth &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_5_gt.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_6_gt.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_45_gt.png} \\
%     % \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_106_gt.png} \\

%     Vanilla NeRF &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/VanillaOcc_5_crop.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/VanillaOcc_6_crop.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/VanillaOcc_44_crop.png} \\
%     % \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/VanillaOcc_106_crop.png} \\

%     RANRAC &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_5_crop.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_6_crop.png} &
%     \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_44_crop.png} \\
%     % \includegraphics[width=.12\textwidth]{images/nerf_artifacts_removed/RANSAC_106_crop.png}
% \end{tabular}
%     \vspace{-0.5cm}
%     \caption{The occlusions lead to well-visible artifacts in the reconstructions of NeRF, these artifacts are completely removed by RANRAC.}
%     \label{fig:nerf_floaters_removed}
%     \vspace{-0.3cm}
% \end{figure}


\begin{figure}
    \centering    
%    \setlength{\wid}{0.23\textwidth}
%    \setlength{\mrg}{-0.2cm}
%    \setlength{\mrgv}{-0.05cm}
%    \begin{tabular}{cc cc}
%        \vspace{\mrgv}
%        \includegraphics[width=\wid]{images/nerf_crops/nerf_6.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/rob_6.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/ours_6.png} & 
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/gt_6.png} 
%        \\  
%        \vspace{\mrgv}
%        \includegraphics[width=\wid]{images/nerf_crops/nerf_25.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/rob_25.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/ours_25.png} & 
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/gt_25.png} 
%        \\ \vspace{\mrgv}
%        \includegraphics[width=\wid]{images/nerf_crops/nerf_47.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/rob_47.png} &
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/ours_47.png} & 
%        \hspace{\mrg}
%        \includegraphics[width=\wid]{images/nerf_crops/gt_47.png} 
 %       \\ 
 %       \vspace{\mrgv}
 %       NeRF & \hspace{\mrg}
%        RobustNeRF & \hspace{\mrg}
%        Ours & \hspace{\mrg}
%        Ground Truth 
%    \end{tabular}
    % \vspace{-0.2cm}
\includegraphics[width=\linewidth]{images/CompactComparison.png}
    \caption{The occlusions lead to well-visible artifacts in the reconstructions of NeRF, these artifacts are completely removed by RANRAC.
    \todo{expand with more quali results for other inconsistencies and datasets}}
    \label{fig:nerf_floaters_removed}
\end{figure}

==> figures/nerf_table.tex <==
\begin{table}[]
    \setlength\tabcolsep{3pt}
    \small
    \centering
    \begin{tabular}{c||ccc|ccc}
        {} &
        \multicolumn{3}{c|}{Mild} &
        \multicolumn{3}{c}{Heavy} \\
        {} &
        PSNR $\uparrow$ &
        $P_5 \uparrow$ &
        $P_1 \uparrow$  &
        PSNR $\uparrow$ &
        $P_5 \uparrow$ &
        $P_1 \uparrow$  \\
        \hhline{=#===|===}
        RANRAC &
        \textbf{27.11} &
        \textbf{25.99} &
        \textbf{25.07} &
        \textbf{26.12} &
        \textbf{24.94} &
        \textbf{24.44} \\

        RobustNeRF &
        26.83 &
        25.58 &
        23.66 &
        25.93 &
        24.79 &
        23.33 \\

        NeRF &
        26.65 &
        22.61 &
        16.74 &
        25.36 &
        18.47 &
        15.97 \\
    \end{tabular}
    \caption{RANRAC achieves state-of-the-art object reconstruction from multiple views. We benchmark against RobustNeRF and NeRF (without any method for robustness) on the watering pot dataset. We compare with milder (10\%) and heavier (17.5\%) amounts of inconsistent perspectives.  All three variants are built on top of instant-nsr for an isolated fair comparison of the robustness method. We report the average PSNR (higher is better) across views. As artifacts introduced by occlusions only contaminate some views, we also report the lower percentiles. RANRAC improves the PSNR significantly compared to NeRF and slightly compared to RobustNeRF.}
    \label{tab:nerfranracquanti}
\end{table}
